Effect of curvature and normal forces on motor regulation of cilia

Cilia are ubiquitous organelles involves in eukaryotic motility. They are long, slender, and motile protrusions from the cell body. They undergo active regular oscillatory beating patterns that can propel cells, such as the algae Chlamydomonas, through fluids. When many cilia beat in synchrony they can also propel fluid along the surfaces of cells, as is the case of nodal cilia. The main structural elements inside the cilium are microtubules. There are also molecular motors of the dynein family that actively power the motion of the cilium. These motors transform chemical energy in the form of ATP into mechanical forces that produce sliding displacement between the microtubules. This sliding is converted to bending by constraints at the base and/or along the length of the cilium. Forces and displacements within the cilium can regulate dyneins and provide a feedback mechanism: the dyneins generate forces, deforming the cilium; the deformations, in turn, regulate the dyneins. This feedback is believed to be the origin of the coordination of dyneins in space and time which underlies the regularity of the beat pattern. Goals and approach. While the mechanism by which dyneins bend the cilium is understood, the feedback mechanism is much less clear. The two key questions are: which forces and displacements are the most relevant in regulating the beat? and how exactly does this regulation occur? In this thesis we develop a framework to describe the spatio-temporal patterns of a cilium with different mechanisms of motor regulation. Characterizing and comparing the predicted shapes and beat patterns of these different mechanisms to those observed in experiments provides us with further understanding on how dyneins are regulated. This comparison is done both, with a linear model that can be analytically solved, as with a non-linear model that we solve numerically.

==> motors_oldnotation.tex <==
\begin{savequote}[75mm] 
euler bernoulli beam quote
\qauthor{Antoni van Leeuwenhoek, 1713} 
\end{savequote}
	
\chapter{Dynamics of collective motors}
\thispagestyle{firststyle}

\newthought{The beat of cilia is powered by the action of molecular motors.} In this chapter we introduce a mesoscopic description of the motor force, and show how oscillatory instabilities  emerge as a collective property of molecular motors. We also introduce a minimal stochastic motor model, and show how regulation via curvature or normal forces can give raise to static circular bends, in agreement with experimental observation.


\section{Nonlinear response of the motor force}
\label{sec:motors}

Consider that a cilium is dynamically bent. Its mechanical properties such as the sliding $\Delta$,  curvature $\dot{\psi}$ and normal force $f_\perp$ will then depend on time. In such a scenario, the motor force can be generically characterized by the non-linear response to the  properties of the cilium. This simply reflects the  idea that motors can dynamically respond to the mechanics of the cilium. For example, in the case in which motors are regulated by the sliding of the doublets, we will have 
\begin{align}
\label{eq:nonlinres}
f_{\rm m}(s,t)&=\lambda^{(0)}+\int_{-\infty}^{\infty}\lambda^{(1)}(t-t')\Delta(s,t')\d t'+\int_{-\infty}^{\infty}\lambda^{(2)}(t-t',t-t'')\Delta(s,t')\Delta(s,t'')\d t'\d t''\nonumber\\
&+\int_{-\infty}^{\infty}\lambda^{(3)}(t-t',t-t'',t-t''')\Delta(s,t')\Delta(s,t'')\Delta(s,t''')\d t'\d t''\d t'''+\ldots\quad ,
\end{align}
where terms of order higher than cubic have not been included. Note that the response kernels $\lambda^{(h)}$ do not depend on arc-length, as the motor properties are assumed to be homogeneous over the cilium. For periodic dynamics the response equation becomes simpler in Fourier space,  where we have
\begin{align}
f_{{\rm m},j} = \lambda^{(0)}+\lambda^{(1)}_{j}\Delta_j+ \lambda^{(2)}_{k,j-k}\Delta_k\Delta_{j-k}+ \lambda^{(3)}_{k,l,j-k-l}\Delta_k\Delta_l\Delta_{j-k-l}+\ldots
\end{align}
with the response coefficients $\lambda^{(h)}_{i,j,k,\ldots}$ being the $h-$dimensional Fourier transform of the corresponding $h-$order kernel. The response coefficients $\lambda^{(h)}_{i,j,k,\ldots}$ completely the motor-filament interaction, and some examples are given in \ref{sec:effmot} and \ref{sec:biochem}.

%The minus sign convention on the left hand side is used so that, for a passive response, the signs of the real and imaginary part of $\lambda^{(1)}$ are positive, as corresponds to a passive spring-dashpot. When real and imaginary part of $\lambda^{(1)}$ become negative then the response is active. 

 
Analogous equations can be written for other motor regulatory mechanisms such as curvature or normal force control. For example, in the case of curvature regulating the motor force we will have
\begin{align}
f_{{\rm m},j} =\beta^{(0)}+\beta^{(1)}_{j}\dot{\psi}_j+ \beta^{(2)}_{k,j-k}\dot{\psi}_k\dot{\psi}_{j-k}+ \beta^{(3)}_{k,l,j-k-l}\dot{\psi}_k\dot{\psi}_l\dot{\psi}_{j-k-l}+\ldots\quad ,
\label{eq:respcurv}
\end{align}
and in the case of normal force control we have 
\begin{align}
f_{{\rm m},j} =\gamma^{(0)}+\gamma^{(1)}_{j}f_{\perp,j}+ \gamma^{(2)}_{k,j-k}f_{\perp,k}f_{\perp,j-k}+ \gamma^{(3)}_{k,l,j-k-l}f_{\perp,k}f_{\perp,l}f_{\perp,j-k-l}+\ldots\quad ,
\label{eq:respnorm}
\end{align}
The response coefficients $\lambda^{(h)}_{i,j,k,\ldots}$ are properties of the motor -filament interactionwhere the response coefficients will be noted $\beta^{(h)}_{i,j,k,\ldots}$ for curvature control throughout this thesis. The usage of $\lambda^{(h)}_{i,j,k,\ldots}$ for sliding control will also be preserved, and the response coefficients to normal force will be noted $\gamma^{(h)}_{i,j,k,\ldots}$

\begin{SCfigure}[\sidecaptionrelwidth][ht]
\includegraphics{./figures/genmod/forvel}	
 	\caption{\textbf{Force-velocity curve of molecular motors.} For values of the control parameter $\Omega$ in the region $\Omega<\Omega_{\rm c}$ the force velocity curve is stable, and motors move at a collective velocity $v_0$. At the critical value $\Omega=\Omega_{\rm c}$ the instability occurs, and finally in the region $\Omega>\Omega_{\rm c}$ the system is unstable.  For  Eq.~\ref{eq:moteff} we have $\Omega=\alpha_1$, and $v_0=0$.}
 	\label{fig:forvel}
\end{SCfigure}



\section{Oscillatory instability of sliding filaments with motors}
\label{sec:effmot}
A collection of molecular motors can cooperate to produce collective behavior such as  spontaneous motion \cite{julicher_cooperative_1995} or oscillatory instabilities \cite{julicher_spontaneous_1997}. To show this, we consider a simple motor model in which the motor force responds to the local sliding velocity of filaments. In particular, we consider the following model
\begin{align}
\partial_t f_{\rm m} = -\frac{1}{\tau_0}(f_{\rm m} - \alpha_1\partial_t \Delta + \alpha_3(\partial_t\Delta)^3)\quad ,
\label{eq:moteff}
\end{align}
where the model parameters are the relaxation time $\tau_0$, the response parameter $\alpha_1$, and the saturation strength $\alpha_3>0$ (the quadratic term is null to preserve time-reversal symmetry). The response coefficients of this model can be easily calculated, and are {\bf check}
\begin{align}
\label{eq:slidresp}
\lambda^{(1)}_{j}=\frac{\alpha_1i\omega j}{1+i\omega j \tau_0}\quad {\rm and}\quad \lambda^{(3)}_{j,k,l}=\frac{\alpha_3i\omega^3jkl}{1+i\omega\tau_0(j+k+l)}\quad,
\end{align}
with $\omega=2\pi/T$ the fundamental angular frequency and $T$ the period. 


At the steady state in which the sliding velocity  $\partial_t\Delta$ is stationary, this model is characterized by a non-linear force velocity relation schematized in Fig.~\ref{fig:forvel}, in which $\Omega=\alpha_1$ is the control parameter. While for values $\alpha_1\le0$ the force-velocity is stable, for  $\alpha_1>0$ there is a region of instability, suggesting that oscillatory instabilities may occur (see Fig.~\ref{fig:forvel}). To see that this is the case consider a very stiff cilium, with $\kappa\to\infty$. In this limit bending and fluid forces are not relevant, and setting the basal stiffness and viscosity to zero, the filament will remain straight (thus $\dot{\psi}=0$). The internal sliding forces are then balanced, and we have 
\begin{align}
f_{\rm m}-k\Delta-\xi_i\partial_t\Delta=0\quad.
\label{eq:forbal}
\end{align}
Together with the motor model  in Eq.~\ref{eq:moteff}, this equation defines a dynamical system. To see how this system can exhibit an instability, consider as {\it ansatz} small perturbations of force and sliding which are $\propto \exp(\sigma t)$. In general $\sigma=\tau^{-1}+i\omega$ is complex, with  $\tau$  the characteristic relaxation time of the perturbation, and   $\omega$ the frequency. Replacing this {\it ansatz}  in the equations one obtains for $\sigma$ the following second order characteristic equation
\begin{align}
\sigma=(k+\xi_{\rm i}\sigma)(1+\tau_0\sigma)/\alpha\quad,
\label{eq:motchar}
\end{align}
which, since it's a complex equation, has just one solution.

\begin{figure}
\includegraphics[width=\textwidth]{./figures/genmod/critical}	
 	\caption{\textbf{Oscillatory instability of motor force.} \textbf{A}. For values of the control parameter $\alpha_1<\alpha_{\rm c}$ the system is stable and shows damped oscillations. \textbf{B}. At the critical point $\alpha_1=\alpha_{\rm c}$ sinusoidal oscillations occur. \textbf{C}. Far from the critical point $\alpha_1>\alpha_{\rm c}$ non-linear oscillations occur, with higher harmonics and a different frequency to that of critical sinusoidal oscillations. In this example, triangular waves. The parameters used for this numerical integration of Eqs.~\ref{eq:moteff}\&\ref{eq:forbal} are $k=1812\,\pN/\um^{2}$, $\xi_{\rm i}=9.76\,\pN\s/\um^2$, $\tau=0.00378\,{\rm s}$, $\alpha_1=\{15,17.6,30\}\,\pN\,\s/\um^2$ and $\alpha_3=4\cdotp10^{-3}\,\pN\,\s^3/\um^4$. The same initial sliding was used in all cases, and the axes of all three panels are equal.}
 	\label{fig:critmot}
\end{figure}

Using the coefficient $\alpha_1$ as control parameter, we can now study the stability of this dynamical system. In particular, note that for $\alpha_1=0$ the system is clearly stable and non-oscillatory, and so $\tau<0$  while $\omega=0$. As $\alpha_1$ increases the system will still be stable (i.e. $\tau<0$), but since $\omega\neq0$ it will exhibit damped oscillations as shown in Fig~\ref{fig:critmot}A. Eventually, the control parameter may reach a critical value $\alpha_{\rm c}$ for which one of the two solutions to Eq.~\ref{eq:motchar} becomes critical, that is $\tau=0$. In this case small amplitude sinusoidal oscillations appear with frequency $\omega$, as can be seen in Fig.~\ref{fig:critmot}B. Finally, for values beyond the critical one (the region $\alpha_1>\alpha_{\rm c}$) non-linear oscillations occur. Their  amplitude is set by the nonlinear saturation term $\alpha_3$, see Fig.~\ref{fig:critmot}C.


Similar models can be devised for curvature and normal force control. In such cases, however, the dynamics of the motor model can not be studied independently from those of the filaments. It is indeed this coupling between the motor force and filaments, together with the dynamic instability of the motor force, which underlies the ciliary beat. An example of a model in which the motor force responds to changes in curvature is 
\begin{align}
\partial_t f_{\rm m} = -\frac{1}{\tau_0}(f_{\rm m} - \alpha_1\dot{\psi} + \alpha_3\dot{\psi}^3)\quad .
\label{eq:moteffcc}
\end{align}
Here  $\tau_0$ corresponds to a delay, $\alpha_1$ to the linear response, and $\alpha_3$ to the saturation which controls the amplitude. The response coefficients in this case are given by \begin{align}
\label{eq:slidresp}
\beta^{(1)}_{j}=\frac{\alpha_1 j}{1+i\omega j \tau_0}\quad {\rm and}\quad \beta^{(3)}_{j,k,l}=\frac{\alpha_3\omega^2jkl}{1+i\omega\tau_0(j+k+l)}\quad.
\end{align}




\section{A minimal biohemical model of ciliary motors}
\label{sec:biochem}
So far we have considered an effective description of the motor force, we now introduce a simple biochemical model capable of giving active response to sliding, curvature, and normal force. To do so, we first note that in the description of the axoneme as a pair of opposing filaments, motors are present in filament A and filament B (see Fig.~\ref{fig:2dgeometry}). The motors rigidly attached to filament B exert with their stalks a force per motor $F_{\rm B}$ on filament A during their power stroke, and a reaction force $−F_{\rm B}$ in filament B. The analogous holds for motors attached to A. Since motors can stochastically attach and detach from the filaments, at a given instant in time there are probabilities $p_{\rm A}$ and $p_{\rm B}$ of a motor being attached to either filament. Thus, given linear motor densities $\rho_{\rm A}$ and $\rho_{\rm B}$ along the two filaments, the total motor force exerted on filament A is
\begin{align}
f_{\rm m} = \rho_{\rm B}p_{\rm B}F_{\rm B}-\rho_{\rm A}p_{\rm A}F_{\rm A}\quad ,
\end{align}
and analogously filament B is subject to a force $-f_{\rm m}$. 

In steady state where motors are stalled the motor force is $F_{\rm A}=F_{\rm B} = F_{\rm st}$, where $F_{\rm st}$ is the stall force. When the motors are moving at a certain velocity, they are characterized by a force-velocity relationship, which we consider for simplicity to be linear with slope $\alpha$. Thus for the motors in filament A we have 
\begin{align}
F_{\rm A} = F_{\rm st} -\alpha\partial_t\Delta_{\rm A}\quad,
\label{eq:singmotofr}
\end{align}
where we note that $\alpha\ge0$ acts as an active friction. Analogously, the force generated by the antagonistic motors is  $F_{\rm B} =F_{\rm st} + \alpha\partial_t\Delta_{\rm B}$. Since $\Delta_{\rm A}=\Delta$ and $\Delta_{\rm B}=-\Delta$ (see \ref{sec:geo}), we can write for the net motor density the following relation
\begin{align}
f_{\rm m} = (\rho_{\rm A}p_{\rm A}-\rho_{\rm B}p_{\rm B})F_{\rm st}+ (\rho_{\rm A}p_{\rm A}+\rho_{\rm B}p_{\rm B})\alpha\partial_t\Delta \quad .
\label{eq:biomot}
\end{align}
Considering the densities of motors to be homogeneous along the filaments, the description of the motor force is complete with the binding kinetics of the motors.

Since motors can either be bound and exerting force or unbound, we have for the motors in filament A the following equation
\begin{align}
\frac{\d p_{\rm A}}{\d t} = -k_{\rm off,A}p_{\rm A} + k_{\rm on}(1-p_{\rm A})
\end{align}
and an analogous one for motors in filament B. It is known that the detachment rate of a molecular motor can be enhanced by the forces which they sustain, and the dependence is exponential according to Bell's law \cite{bell_models_1978}. If we generalize this to also allow curvature dependent detachment, we have
\begin{align}
k_{\rm off,A} = k_0 \exp\left[\frac{F_{\rm A}}{F^{\rm c}} + \frac{f_\perp}{f_{\perp}^{\rm c}}+ \frac{C_{\rm A}}{C^{\rm c}}\right]\quad ,
\label{eq:bell}
\end{align}
where $F^{\rm c}$ is the characteristic sliding detachment force, $f_\perp$ is the compressive force as defined  in Eq.~\ref{eq:dynfor}, $f_{\perp}^{\rm c}$  the characteristic spacing detachment force, and $C^{\rm c}$ the characteristic detachment curvature. Together Eqs.~\ref{eq:biomot}-\ref{eq:bell} are a minimal biochemical description of this motor model. Just as the effective description introduced in \ref{sec:effmot}, this biochemical model of opposing motors exhibits sliding oscillations for rigid filaments. 

\begin{figure}
\includegraphics[width=\textwidth]{./figures/genmod/opposing.pdf}	
 	\caption{\textbf{Sliding oscillations of antagonistic biochemical motors.} \textbf{A}. The  probabilities of the motors in the rigid filaments A and B to be bound oscillate with a phase shift. \textbf{B}. The mismatch in binding probability generates a net active motor force $f_{\rm m}$, which is also oscillatory. \textbf{C}. This finally results in sliding oscillations. The parameters used for this numerical integration of Eqs.~\ref{eq:biomot}\&\ref{eq:bell} are $k=1812\,\pN/\um^{2}$, $\xi_{\rm i}=9.76\,\pN\s/\um^2$, $k_{\rm on}=14\,\s^{-1}$, $k_0=2.3\,\s^{-1}$, $\alpha=0.04$, $\rho_{\rm A}=\rho_{\rm B}=10^3\,{\rm motors}/\um$, $F^{\rm c}=1\,\pN$, and $F_{\rm st}=4\,\pN$. }
 	\label{fig:critmot}
\end{figure}

In the static regime, the motors are stalled, and the motor force density takes the value
\begin{align}
f_{\rm m}=(\rho_{\rm A}-\rho_{\rm B})p_{\rm 0}F_{\rm st}\quad,
\label{eq:motstat}
\end{align}
where $p_0$ is the stall attachment probability which in the limit $C_{\rm A}=C_{\rm B}=\dot{\psi}$ of constant spacing (see Eq.~\ref{eq:curvAB}) is the same for motors on both filaments. This static attachment probability is given by 
\begin{align}
p_0 = \left(1+\frac{k_0}{k_{\rm on}}\exp\left[\frac{F_{\rm st}}{F^{\rm c}} + \frac{f_{\perp,0}}{f_{\perp}^{\rm c}}+ \frac{\dot{\psi}_0}{C^{\rm c}}\right]\right)^{-1}\quad ,
\label{eq:motstat}
\end{align}
and is independent of the static sliding, but depends on the static curvature and normal force raising the possibility of static regulation of bent shapes. Importantly, the static motor force vanishes for the case $\rho_{\rm A}=\rho_{\rm B}$. Thus in this model static active force can only be generated when lateral symmetry  is broken.

Following the prescriptions of the previous section, the response coefficients of the motor force to sliding, curvature, and normal forces can be calculated order by order. In particular, the linear coefficients are
\begin{align}
\label{eq:motres}
\lambda^{(1)}_n&= -(\rho_{\rm A}+\rho_{\rm B})p_0(1-p_0)\frac{i\omega n+(\omega n)^2p_0/k_{\rm on}}{1+(\omega n p_0/k_{\rm on})^2}\frac{F_{\rm st}}{F^{\rm c}}\alpha+(\rho_{\rm A}+\rho_{\rm B})p_0\alpha i\omega n\nonumber\\
\beta^{(1)}_n&=(\rho_{\rm A}-\rho_{\rm B})p_0(1-p_0)\frac{1-i\omega n p_0/k_{\rm on}}{1+(\omega n p_0/k_{\rm on})^2}\frac{F_{\rm st}}{C^{\rm c}}\nonumber\\
\gamma^{(1)}_n&=(\rho_{\rm A}-\rho_{\rm B})p_0(1-p_0)\frac{1-i\omega n p_0/k_{\rm on}}{1+(\omega n p_0/k_{\rm on})^2}\frac{F_{\rm st}}{f_\perp^{\rm c}}
\end{align}
Importantly, for the case $\rho_{\rm A}=\rho_{\rm B}$ in which lateral symmetry is preserved, the response coefficients to curvature and normal force vanish ($\beta^{(1)}_j=\gamma^{(1)}_j=0$), but the one to sliding does not (this is only true in the limit $a\to a_0$, otherwise curvature control would produce a response to spacing). On the other hand, in the case that $\rho_{\rm A}\neq\rho_{\rm B}$ this model exhibits static regulation if it is sensitive to curvature and normal forces, since according to Eq.~\ref{eq:motstat} $p_0$ will be  a function of arc-length. In this case the linear response coefficients above will not be homogeneous along the arc-length. Finally, we note that in the sliding response coefficient only the second term is active, with the first one corresponding to protein friction.



\section{Motor regulation produces circular bends}
\label{sec:circles}
In section \ref{sec:minreq} we saw that the shapes resulting from a constant motor force in the cilium is a linear decrease of curvature, which corresponds to a spiral shape. The presence of cross-linkers makes the decay of curvature even faster (see Fig.~\ref{fig:statminreq}). However, we described in section \ref{sec:circles} experiments where the shapes of statically bent doublets were circular arcs. That is, they were characterized by a linearly growing tangent angle and thus a constant curvature (see Fig.~\ref{fig:bendtrack}). This suggests  motor regulation as that introduced in this chapter is playing a role in producing a non-homogeneous distribution of bound motors.


\begin{figure}[h]
\centerline{\includegraphics[width=\textwidth]{./figures/statics/regulation}}
\caption{\textbf{Formation of arcs under force regulation.}  A uniform force distribution (panel A, red curve) produces a spiral shape (panel B, red curve). Tip-concentrated force distributions (panel A, yellow and blue curves) produce nearly circular arcs (panel B, yellow and blue curves).}
\label{fig:circsketch}
\end{figure}

We can infer the distribution of the active motors from the shape using the moment balance equation (Eq.~\ref{eq:stat}), which after one integration is $F(s)=\kappa C(s)/a_0$. This balance equation implies that the motor activity is concentrated at the distal end of the filaments pair, $s=L$. This follows because a circular arc (i.e., a shape with constant curvature) requires a constant total force, which in turn requires the sliding force density $f(s)$ to be zero except at the distal end. Indeed, in Fig.~\ref{fig:circsketch}A we show three examples of motor force distributions, with the corresponding shapes in Fig.~\ref{fig:circsketch}B obtained from numerically solving Eq.~\ref{eq:stat}. As the motor force accumulates more at the tip of the cilium, the shape becomes closer to a circular arc.

To obtain such circular shapes we consider the biochemical model from the previous section in the static limit. In this case there is no sensitivity to sliding, as $\partial_t\Delta=0$, but motors can sense curvature and normal forces. The moment balance Eq.~\ref{eq:stat} together with Eq.~\ref{eq:motstat} for the motor binding probability results in
\begin{align}
\kappa\ddot{\psi}(s) = -\frac{ \rho_{\rm A}a_0F_{\rm st} }{1+u\exp\left[\left(\frac{\dot{\psi}(s)}{\sqrt{a_0F^{\rm c}_\perp/\kappa}}\right)^2+\frac{\dot{\psi}(s)}{C^{\rm c}}\right]}\quad .
\label{eq:vikram}
\end{align}
where we have used that the normal force is given by $f_\perp=\dot{\psi}^2/a_0$ and that $\rho_{\rm B}=0$, since in the doublet experiment only the motors of one filament are exerting active forces. We have also defined the parameter $u = k_0\exp[F_{\rm st}/F^{\rm c}]/k_{\rm on}$, which is the fraction of time that the motor spends unbound. This equation leads to force concentration at the distal end, as can be seen by the following argument.

Motor sliding forces cause bending, which results in a normal force that tends to separate the filament pair. When the normal force $f_\perp(s)$ exceeds the characteristic normal force density $F_{\rm c}$, the motors detach, resulting in a decrease in sliding force. Only near the distal end, at which the curvature decreases to zero (according to the boundary condition in Eq.~\ref{eq:bcstatuse}), will the normal force fall below its critical value and the motors will remain attached. Thus, this motor regulation mechanism results in feedback: as the doublet starts to bend, the higher curvature at the base (Fig.~\ref{fig:circsketch}) causes basal motors to detach, and as the bend develops there will be a wave of detachment that only stops at the distal end. Note that this argument is equally valid for normal force and curvature regulation.

\subsection{Comparison to disintegrated doublet experiments}
To compare quantitatively the predictions of this model with the experimental data, we numerically integrated Eq.~\ref{eq:vikram} using the boundary conditions in Eq.~\ref{eq:bcstatuse}. For regulation via normal force, which is shown in yellow in Fig.~\ref{fig:bendreg}, we use as  parameters a stall motor force $F_{\rm st}=5\,\pN$, a motor density $\rho_{\rm A}=200\,\um^{-1}$, a bending stiffness $\kappa=120\,\pN\,\um^{2}$, a critical-motor force $f^{\rm c}_\perp=200\,\pN/\um$ and no curvature control $C^{\rm c}\to\infty$.  For the solution under curvature control which is shown in blue, we use the same parameters but a critical curvature of $C^{\rm c}=0.18\um^{-1}$ and  no normal force regulation by setting $f^{\rm c}_\perp\to\infty$. In both cases we consider $u=0.1$.


\begin{figure}[h]
\centerline{\includegraphics[width=\textwidth]{./figures/statics/comparison.pdf}}
\caption{\textbf{ Comparison of model and tracked data.} \textbf{A.} Tangent angle vs arc-length for several control mechanisms. Red line corresponds to no control (or sliding control), yellow to normal force control,  and blue to curvature control. Dots correspond to tracked data, note that no control departs significantly from the data. \textbf{B.} Curvature vs arc-length for three control mechanisms. The data, which is noisier than in A, shows a roughly constant curvature that decreases towards the end. Normal force control (yellow) and curvature control (blue)  show the same behavior, but no control (in red) does not.}
\label{fig:bendreg}
\end{figure}

As we can see in Fig.~\ref{fig:bendreg}, these two regulatory mechanisms (in blue and yellow) give raise to shapes in which the tangent angle increases roughly linearly, as corresponds to a constant curvature. They both show good agreement with the experimental data (black circles), and are clearly different from the case of no regulation, in which the angle increases parabolically (red lines). We mention now that the forces and shapes in Fig.~\ref{fig:circsketch} correspond to these solutions. That is, normal-force and curvature regulation concentrates the forces at the distal tip. In this region where motors are attached, there is a sharp decrease of the curvature, which is zero at the end of the filament (Fig.~\ref{fig:bendreg}B).

If there is no regulation by normal force or curvature, then all motors will have the same probability of being attached, resulting in a constant force per unit length. As already discussed, this results in a linearly decreasing curvature (see Figs.~\ref{fig:circsketch} and \ref{fig:bendreg}, red lines), which is not consistent with the experimental data. The sliding control model, where detachment is proportional to the sliding force experienced by the motors (given by Eq.~\ref{eq:singmotofr}), also leads to a constant force density because, at steady state, the shear force experienced by all the motors is the same, and corresponds to the stall force. Thus, the sliding control model also has a constant shear force per unit length, and, like the unregulated case, leads to a non-circular shape, inconsistent with the observations.

\begin{SCfigure}[\sidecaptionrelwidth][h!]
\includegraphics[width=.5\textwidth]{./figures/statics/curvlen}	
 	\caption[Swimming path of the axoneme.]{\textbf{Dependence of average curvature on filament length.} The curvatures of the five tracked split axonemes (insets) show a weak dependence on their length (green symbols). Curvature control (blue line) and normal-force control (yellow line) both predict the observed weak length dependence, without introducing additional parameters. In the absence of regulation, the predicted linear scaling vastly deviates from the data (red line).}
 	\label{fig:curlen}
\end{SCfigure}


To determine how curvature depends on filament length, we analyzed five pairs of microtubule doublets that showed the arcing behavior whose lengths ranged from 5 to 9 $\um$. A total of 24 arcing events were observed, with up to 8 events for a single pair of filaments. All bent into nearly circular arcs (Fig.~\ref{fig:curlen}, upper images). The average curvature (excluding the last 1 $\um$ from the distal tip) increased only weakly with the length of the doublets (Fig.~\ref{fig:curlen}, filled points). The same parameters used in Fig.~\ref{fig:bendreg} were then used to fit the curvature vs. length data for all five doublet pairs, without any additional parameters. Both the curvature control and the normal-force control models were in very good agreement with the data (Fig.~\ref{fig:curlen}, blue and yellow curves respectively). The models predict a weak dependence of the curvature on filament length because it is only the most-distal motors that generate the bending forces. By contrast, if the density of active motors were constant along the doublets, as in the sliding control model, then the average curvature would be proportional to length (integrating Eq. 3), which is inconsistent with the data (Fig.~\ref{fig:curlen}, red line).

%
%\section{Conclusions}
%\begin{itemize}
%\item {\bf Minimal requirements for bending:} summarize. possibility of experimental verification, straightening of bent axonemes
%\item {\bf Role of cross-linkers}
%\item {\bf Static motor regulation produces circular arcs: } On the other hand, 
%\end{itemize}
%



==> statics.tex <==
\begin{savequote}[75mm] 
euler bernoulli beam quote
\qauthor{Antoni van Leeuwenhoek, 1713} 
\end{savequote}
	
\chapter{Motor regulation in statically bent filaments}
\thispagestyle{firststyle}

\newthought{In order to understand the mechanism regulating the shapes of the axoneme,} we begin by analyzing the static limit. In particular, we  analyze the requirements to bend an axoneme and the effects of motor regulation on its shape. We finalize by comparing our predictions with experimental results.

\section{Static equilibrium of an isolated axoneme}
\label{sec:statuse}
In section \ref{sec:stat} we introduced the equations of static equilibrium for a pair of opposing filaments under external and internal sliding forces. Here we focus on the case in which there are no external forces, and thus bending must arise by the effect of motors producing a static sliding force $f_{\rm m}$ as described in \ref{sec:biochem}\footnote{Since throughout this section we will only consider static shapes, we will drop the sub-index 0 to denote the zeroth Fourier mode of quantities.}

In particular, we  focus on the case of homogeneous spacing  $a\to a_0$. This requires that $k_\perp\to\infty$, while keeping the normal force  $f_\perp=k_\perp(a-a_0)$ finite, such that it acts as a Lagrange multiplier. In this regime we have that the equilibrium equations \ref{eq:allstat}  become
\begin{align}
0&=\partial_s\left[ (\kappa\ddot{\psi}  + a_0 f){\bf n}-\tau{\bf t} \right]\nonumber\\
f_\perp&=F\dot{\psi}\nonumber\\
 k_0\Delta_0&=F(0)\quad ,
 \label{eq:staticuse}
\end{align}
where as introduced in Eq.~\ref{eq:statfor} the sliding force density is  $f=f_{\rm m}-k\Delta$, and $F=\int_?^? f$  is the net sliding force. Note that the normal force $f_\perp$ is directly given from the filament shape and its internal force, and does not appear elsewhere. The relationship between sliding and geometry in this case is \ref{sec:simplegeo}
\begin{align}
\Delta(s)=\Delta_0+a_0(\psi(s)-\psi(0))\quad .
\label{eq:slidingagain}
\end{align}
Finally, the boundary balance equations in Eqs.~\ref{eq:fullbc}  simplify to
\begin{align}
\label{eq:staticbcuse}
(\kappa\ddot{\psi}(0) + a_0 f(0)){\bf n}(0)-\tau(0){\bf t}(0)&=0\nonumber\\
(\kappa\ddot{\psi}(L)+ a_0 f(L)){\bf n}(L)-\tau{\bf t}(L)&=0 \nonumber\\
\kappa\dot{\psi}(0)-a_0k_0\Delta_0&=0\nonumber\\
\dot{\psi}(L)&=0\quad .
\end{align}
Together Eqs.~\ref{eq:staticuse}-\ref{eq:staticbcuse} define a boundary value problem which, provided the motor force, can be solved.

Integrating the first line in Eq.~\ref{eq:staticuse} twice and using the first two boundary conditions to fix the integration constants, one obtains that the tension is null (that is, $\tau(s)=0$), and that the moment balance simplifies to
\begin{align}
\kappa\ddot{\psi}(s) &=- a_0f(s) 
\label{eq:stat}
\end{align}
This equation is invariant under rotations, that is the addition of a global constant angle. We arbitrarily choose a reference frame for which $\psi(0)=0$. Using further the third boundary condition in this moment balance gives $a_0 F=\kappa\dot{\psi}$, from which we obtain that the spacing force density is given by
\begin{align}
f_\perp= \kappa \dot{\psi}^2/a_0
\end{align} 
Note that because $f_\perp(s)$ is always positive, curvature always tends to separate the two filaments. The remaining boundary balance and  rotational invariance give the  two boundary conditions
\begin{align}
\kappa\dot{\psi}(0)=a_0k_0\Delta_0\quad {\rm and}\quad \psi(0)=0\quad ,
\label{eq:bcstatuse}
\end{align}
which together with Eq.~\ref{eq:slidingagain} and provided a motor force model, allow solving the moment balance in  Eq.~\ref{eq:stat}. We now study different solutions of this static problem.

\section{Minimal requirements for static bending}
\label{sec:minreq}
To proceed further we need to consider a motor model. Here we use the static limit of the biochemical motor model introduced in \ref{sec:biochem}. In this model filaments A and B have opposing populations of molecular motors with linear densities $\rho_{\rm A}$ and $\rho_{\rm B}$, whose detachment is enhanced by sliding forces, curvature or normal forces according to Eq.~\ref{eq:bell}. The motor force in the static limit is given by Eq.~\ref{eq:motstat}, with the binding probability $p_0$ of motors given by Eq.~\ref{eq:motstat}.

In the case in which both filaments have the same properties then densities are equal, that is $\rho_{\rm A}=\rho_{\rm B}$. In this case we have that the opposing forces balance each other and $f_{\rm m}^{\rm st}=0$, thus the cilium doesn't bend ($\psi(s)=0$) nor does it slide ($\Delta_0=0$). When $\rho_{\rm A}\neq\rho_{\rm B}$, then  Eq.~\ref{eq:stat} gives non-trivial solutions. The cases of sensitivity to curvature and spacing forces will be studied in the next section, and for now we focus in the limit in which motors are insensitive to these and so $f_{\perp}^{\rm c}\to\infty$ and $C^c\to \infty$.

In this limit the attachment probabilities are  constant over the arc-length of the axoneme, as from Eq.~\ref{eq:motstat} we have
\begin{align}
p_0=\left(1+\frac{k_0}{k_{\rm on}}\exp\left[\frac{F_{\rm st}}{F^{\rm c}}\right]\right)^{-1}\quad .
\label{eq:motnoreg}
\end{align}
We can then solve Eq.~\ref{eq:stat} analytically and obtain
\begin{align}
\psi(s) = \frac{a\ell k_0\Delta_0}{\kappa} \frac{\cosh[L/\ell]-\cosh\left[{(L-s)/\ell}\right]}{\sinh\left[L/\ell\right]}\quad ,
\label{eq:solpsi}
\end{align}
where we have used the two boundary conditions in Eq.~\ref{eq:bcstatuse}, and defined the characteristic length 
\begin{align}
\ell=\sqrt{\kappa/(k a^2)}
\label{eq:charlen}
\end{align}
beyond which the sliding compliance of the motors becomes significant. The basal sliding  $\Delta_0$ is obtained  via  Eq.~\ref{eq:slidingagain}, and is
\begin{align}
\Delta_0 = \frac{ f_{\rm st}}{k + (k_0/\ell)\coth[L/\ell] }\quad ,
\label{eq:solD0}
\end{align}
where we have defined the stalled motor force density as $f_{\rm st}=(\rho_{\rm A}-\rho_{\rm B})p_0F_{\rm st}$, which does not depend on arc-length since $p_0$ is given by Eq~\ref{eq:motnoreg}. Note however that due to the presence of static cross-linkers with stiffness $k$ the net sliding force $f=f_{\rm m}-k\Delta$ does indeed depend on arc-length.


\begin{figure}[!h]
\centerline{\includegraphics{./figures/statics/basal.pdf}}
\caption{\textbf{Role of cross-linkers in bending.} \textbf{A.} For weak cross-linkers we have  $L\gg\ell$, and the resulting shape has a linearly decreasing curvature. As cross-linkers get stronger (values for increasing shades of green are $k=10^{-1}\,\pN/\um^2$, $k=10^2\,\pN/\um^2$ and $k=10^3\,\pN/\um^2$), $L$ becomes comparable and eventually bigger than $\ell$, which flattens the resulting shape. \textbf{B.} Dependence of maximal curvature with cross-linker stiffness for three values of basal compliance. The softer the cross-linkers, the larger the curvature. Decreasing shades of red correspond to $k_0=92352\,\pN/\um$, $k_0=923.5\,\pN/\um$ and $k_0=9.2\,\pN/\um$, and the dots correspond to the curvatures in A. \textbf{C.} Dependence maximal curvature with basal stiffness for three decreasing cross-linker stiffness (decreasing shades of blue correspond to $k=2280\,\pN/\um^2$, $k=228\,\pN/\um^2$ and $k=22.8\,\pN/\um^2$). Stiffer bases result in higher curvatures. \textbf{D.} Three examples of shapes corresponding to the dots in C. Other parameters are  $\kappa= 1730\,\pN\cdotp\um^2$; $L = 30\,\um$; $a = 0.185\,\um$;  $f_{\rm m}=500\,\pN/\um$ and, unless otherwise specified, $k_0 =92352\,\pN/\um $ and $k = 228\,\pN/\um^2$ which gives $\ell\approx 15$.}
\label{fig:statminreq}
\end{figure}


To characterize the static shapes given by Eq.~\ref{eq:solpsi} we first consider the limit in which the role of cross-linkers is small, and thus $L\ll \ell$. To do this, we expand  in $L/\ell$ and obtain
\begin{align}
\psi(s)=-\frac{a_0 f_{\rm st}}{\kappa}\left(\frac{s^2}{2}-sL\right)\quad .
\end{align}
This parabolic solution implies that for filaments of length $L\gg\ell$ the curvature decreases linearly along the arc-length from its maximum value at the base to the minimum at the tip, as is shown in Fig.~\ref{fig:statminreq}A. For shorter filaments the effect of cross-linkers becomes more prominent, which  makes the curvature decrease sub-linearly, and also reduces the maximum curvature at the base.


A key parameter that characterizes the bent cilium is thus its maximal curvature $C_{\rm max}=\dot{\psi}(0)$, which is shown in Fig.~\ref{fig:statminreq}B as a function of $k$ for several values of  $k_0$. The maximal curvature  decreases monotonically as the cross-linkers become stiffer, and saturates for vanishing cross-linker stiffness. At the same time, the maximal curvature increases as the base of the cilium becomes stiffer ($k_0$ grows), and eventually saturates in the limit of an incompressible base for which $\Delta_0=0$ (when $k_0\gg kL$, see Fig. \ref{fig:statminreq}C, and Fig.~\ref{fig:statminreq}D for three examples of shapes). Clearly in this limit the maximal curvature still depends on the bulk cross-linker stiffness  $k$.  In particular, note that for $k_0=0$ there is sliding, $\Delta=f_{\rm m}/k$, but the cilium remains straight, $\psi=0$. Our analysis thus indicates that for the static bending of cilia a basal stiffness is necessary, and the stronger it is the higher the bend.


Until now we have shown that bending requires a lateral asymmetry ($\rho_{\rm A}\neq\rho_{\rm B}$)  and a polar asymmetry which we have described by a basal stiffness ($k_0\neq0$). An alternative way of introducing the polar asymmetry is to remove the basal constrain ($k_0=0$) but consider an inhomogeneous cross-linker stiffness. One possibility is the linear profile $k(s) = \tilde{k}(1-\epsilon s/L)$, with $\epsilon$  the slope of the linear gradient and $\tilde{k}$ the cross-linker stiffness at the base. In this case, one recovers a flat solution when $\epsilon=0$. As the gradient slope grows (see Fig.~\ref{fig:statminreq}C), the bend develops and the maximal curvature increases until it saturates for steep gradients (see Fig.~\ref{fig:grad}). Since a linear gradient is a smaller inhomogeneity than a basal stiffness, the maximal curvature in the limit $L\gg\ell$ is smaller than in the case where a basal stiffness is present (compare Fig.~\ref{fig:grad} to Fig.~\ref{fig:statminreq}A).



\begin{SCfigure}[\sidecaptionrelwidth][h!]
\includegraphics[]{./figures/statics/gradient}	
 	\caption{\textbf{Bending with cross-linker gradient.} The maximal curvature grows with the  cross-linker gradient. Values are as in Fig.~\ref{fig:statminreq}, with increasing shades of green corresponding to $\tilde{k}= 10^{-1}\,\pN/\um^2$, $\tilde{k}=10^2\,\pN/\um^2$ and $\tilde{k}=10^4\,\pN/\um^2$. Here $\ell$ is defined using $k(s=0)$. \label{fig:grad}}
\end{SCfigure}

\section{Motor regulation produces circular bends}
\label{sec:circles}
So far we have considered that motors are not sensitive to normal forces or curvature. In this case, the distribution of bound motors along the axonemal length is homogeneous. The resulting shapes when cross-linkers are weak is a linear decrease of curvature, which corresponds to a spiral shape. The presence of cross-linkers makes the decay of curvature even faster. In section \ref{sec:circles} we described experiments where a protease treatment removed cross linkers between a pair of doublets. The shapes which these doublets obtained quasi-statically were clearly circular arcs. That is, they were characterized by a linearly growing tangent angle and thus a constant curvature (see Fig.~\ref{}). This suggests that some type of motor regulation may be at play, producing a non-homogeneous distribution of bound motors.


\begin{figure}[h]
\centerline{\includegraphics[width=\textwidth]{./figures/statics/regulation}}
\caption{\textbf{Formation of arcs under force regulation:}  A uniform force distribution (panel A, red curve) produces a spiral shape (panel B, red curve). Tip-concentrated force distributions (panel A, yellow and blue curves) produce nearly circular arcs (panel B, yellow and blue curves).}
\label{fig:circsketch}
\end{figure}

We can infer the distribution of the active motors from the shape using the moment balance equation (Eq.~\ref{eq:stat}), which after one integration is $F(s)=\kappa C(s)/a_0$. This balance equation implies that the motor activity is concentrated at the distal end of the filaments pair, $s=L$. This follows because a circular arc (i.e., a shape with constant curvature) requires a constant total force, which in turn requires the sliding force density $f(s)$ to be zero except at the distal end. Indeed, in Fig.~\ref{fig:circsketch}A we show three examples of motor force distributions, with the corresponding shapes in Fig.~\ref{fig:circsketch}B obtained from numerically solving Eq.~\ref{eq:stat}. As the motor force accumulates more at the tip of the cilium, the shape becomes closer to a circular arc.

To obtain such circular shapes we allow for motor regulation via curvature and normal forces. That is, we let $C^{\rm c}$ and $F_\perp^{\rm c}$ in Eq.~\ref{eq:bell} to be finite. In this case, the moment balance Eq.~\ref{eq:stat} together with Eq.~\ref{eq:motstat} for the motor binding probability results in
\begin{align}
\kappa\ddot{\psi}(s) = -\frac{ \rho_{\rm A}a_0F_{\rm st} }{1+u\exp\left[\left(\frac{\dot{\psi}(s)}{\sqrt{a_0F^{\rm c}_\perp/\kappa}}\right)^2+\frac{\dot{\psi}(s)}{C^{\rm c}}\right]}\quad .
\label{eq:vikram}
\end{align}
Here we are considering $\rho_{\rm B}=0$, as in the doublet experiment only the motors of one filament are exerting active forces. We have also defined the parameter $u = k_0\exp[F_{\rm st}/F^{\rm c}]/k_{\rm on}$, which is the fraction of time that the motor spends unbound. This equation leads to force concentration at the distal end, as can be seen by the following argument.

Motor sliding forces cause bending, which results in a normal force that tends to separate the filament pair. When the normal force exceeds the characteristic normal force density, the motors detach, resulting in a decrease in sliding force. Only near the distal end, at which the curvature decreases to zero (according to the boundary condition), will the normal force fall below its critical value and the motors will remain attached. Thus, this motor regulation mechanism results in feedback: as the doublet starts to bend, the higher curvature at the base (Fig.~\ref{fig:circsketch}) causes basal motors to detach, and as the bend develops there will be a wave of detachment that only stops at the distal end. Note that this argument is equally valid for normal force and curvature regulation.

\subsection{Comparison to disintegrated doublet experiments}
To compare quantitatively the predictions of this model with the experimental data, we numerically integrated Eq.~\ref{eq:vikram} using the boundary conditions in Eq.~\ref{eq:bcstatuse}. For regulation via normal force, which is shown in yellow in Fig.~\ref{fig:bendreg}, we use as  parameters a stall motor force $F_{\rm st}=5\,\pN$, a motor density $\rho_{\rm A}=200\,\um^{-1}$, a bending stiffness $\kappa=120\,\pN\,\um^{2}$, a critical-motor force $f^{\rm c}_\perp=200\,\pN/\um$ and no curvature control $C^{\rm c}\to\infty$.  For the solution under curvature control which is shown in blue, we use the same parameters but a critical curvature of $C^{\rm c}=0.18\um^{-1}$ and  no normal force regulation by setting $f^{\rm c}_\perp\to\infty$.


\begin{figure}[h]
\centerline{\includegraphics[width=\textwidth]{./figures/statics/comparison.pdf}}
\caption{\textbf{ Comparison of model and tracked data.} \textbf{A.} Tangent angle vs arc-length for several control mechanisms. Red line corresponds to no control, yellow to normal force control,  and blue to curvature control. Dots correspond to tracked data, not that no control departs significantly from the data. \textbf{B.} Curvature vs arc-length for three control mechanisms. The data, which is noisier than in A, shows a roughly constant curvature which decreases towards the end. Normal force (yellow) and curvature (blue) control show the same behavior, but no control (in red) does not.}
\label{fig:bendreg}
\end{figure}

As we can see in Fig.~\ref{fig:bendreg}, these two regulatory mechanisms (in blue and yellow) give raise to shapes in which the tangent angle increases roughly linearly, as corresponds to a constant curvature. They both show good agreement with the experimental data (black circles), and are clearly different from the case of no regulation, in which the angle increases parabolically (red lines). We mention now that the forces and shapes in Fig.~\ref{fig:circsketch} correspond to these solutions. That is, normal-force and curvature regulation concentrates the forces at the distal tip. In this region where motors are attached, there is a sharp decrease of the curvature, which is zero at the end of the filament (Fig.~\ref{fig:bendreg}B).

If there is no regulation by normal force or curvature, then all motors will have the same probability of being attached, resulting in a constant force per unit length. As already discussed, this results in a linearly decreasing curvature (see Fig.~\ref{fig:circsketch}\&\ref{fig:bendreg}, red lines), which is not consistent with the experimental data. The sliding control model, where detachment is proportional to the sliding force experienced by the motors (given by Eq.~\ref{eq:singmotofr}), also leads to a constant force density because, at steady state, the shear force experienced by all the motors is the same, and corresponds to the stall force. Thus, the sliding control model also has a constant shear force per unit length, and, like the unregulated case, leads to a non-circular shape, inconsistent with the observations.

\begin{SCfigure}
\includegraphics[width=.5\textwidth]{./figures/statics/curvlen}	
 	\caption[Swimming path of the axoneme.]{\textbf{Dependence of average curvature on filament length.} The curvatures of the five tracked split axonemes (insets) show a weak dependence on their length (green symbols). Curvature control (blue line) and normal-force control (yellow line) both predict the observed weak length dependence, without introducing additional parameters. In the absence of regulation, the predicted linear scaling vastly deviates from the data (red line).}
 	\label{fig:curlen}
\end{SCfigure}


To determine how curvature depends on filament length, we analyzed five pairs of microtubule doublets that showed the arcing behavior whose lengths ranged from 5 to 9 $\um$. A total of 24 arcing events were observed, with up to 8 events for a single pair of filaments. All bent into nearly circular arcs (Fig.~\ref{fig:curlen}, upper images). The average curvature (excluding the last 1 $\um$ from the distal tip) increased only weakly with the length of the doublets (Fig.~\ref{fig:curlen}, filled points). The same parameters used in Fig.~\ref{fig:bendreg} were then used to fit the curvature vs. length data for all five doublet pairs, without any additional parameters. Both the curvature control and the normal-force control models were in very good agreement with the data (Fig.~\ref{fig:curlen}, blue and yellow curves respectively). The models predict a weak dependence of the curvature on filament length because it is only the most-distal motors that generate the bending forces. By contrast, if the density of active motors were constant along the doublets, as in the sliding control model, then the average curvature would be proportional to length (integrating Eq. 3), which is inconsistent with the data (Fig.~\ref{fig:curlen}, red line).

%
%\section{Conclusions}
%\begin{itemize}
%\item {\bf Minimal requirements for bending:} summarize. possibility of experimental verification, straightening of bent axonemes
%\item {\bf Role of cross-linkers}
%\item {\bf Static motor regulation produces circular arcs: } On the other hand, 
%\end{itemize}
%


